On the extended nature of edge states of Quantum Hall Hamiltonians

Properties of eigenstates of one-particle Quantum Hall Hamiltonians localized near the boundary of a two-dimensional electron gas - so-called edge states - are studied. For finite samples it is shown that edge states with energy in an appropriate range between Landau levels remain extended along the boundary in the presence of a small amount of disorder, in the sense that they carry a non-zero chiral edge current. For a two-dimensional electron gas confined to a half-plane, the Mourre theory of positive commutators is applied to prove absolute continuity of the energy spectrum well in between Landau levels, corresponding to edge states.

==> paper/details.tex <==
To begin with, we consider the spatial decay of the free 
resolvent $(E-H_0)^{-1}$. This free resolvent 
for a homogeneous magnetic field Hamiltonian in two
dimensions can be calculated using an expansion in eigenfunctions 
of $H_0$, which are known explicitely in terms of Laguerre
polynomials. See \cite{Lehmann} and \cite{JP} for more details. References to
addition theorems for Laguerre polynomials that are useful in the calculation, 
include \cite{EMOT} and, for proofs of the formulae, \cite{Miller}. The result
contains the confluent hypergeometric function called $\Psi$ in the notation
of \cite{EMOT}.
\begin{equation}
\begin{split}
R_0(x,y;E)& =
(E-H_0)^{-1}(r_1e^{i\varphi_1},r_2e^{i\varphi_2}) \\ & =
-\frac{1}{4\pi} e^{i\pi\zeta}\Gamma(-\zeta)e^{ir_1r_2\sin(\varphi_1 -
  \varphi_2)} e^{-\frac{B}{4} (\abs{x-y}^2}
  \Psi\bigl(-\zeta,1;\frac{B}{4}\abs{x-y}^2\bigr)
\end{split}
\end{equation}
$\zeta$ is related to the energy by $E=(2\zeta+1)B$, so that $R_0$ has 
singularities at Landau-band energies. $\Psi(-\zeta,1;z)$ has a
logarithmic singularity at $z=0$ and behaves for large $\abs{z}$ as
$\abs{z}^{\zeta}$. This implies a Gaussian decay for large $\abs{x-y}$. We
will, however, only use an estimate of the form
\begin{equation}
\label{eq:R0}
\abs{R_0(x,y;E)} \leq C e^{-
  \abs{x-y}/\xi} \abs{\ln(\abs{x-y}/\xi)},
\end{equation}
with a decay length scale $\xi$ on the order of the magnetic length
$\sqrt{B}^{-1}$. 

We now include the disorder potential and claim the following 

\begin{lemma}
Let $V_0$ be a not too fast increasing 
edge potential that describes the Corbino-disc with varying
sample size $R$. Let further $V_d$ be bounded by a constant sufficiently small
compared to the magnetic field. Let finally $\Delta$ be an energy intervall in
the gaps of $H_0+V_d$. Then there
are positive constants $C$, $\lambda$, and $a<R$, 
such that an eigenfunction $\psi$ of
$H=H_0+V_0+V_d$ with energy $E\in\Delta$ satisfies
\begin{equation}
\abs{\psi(x)} \le C e^{-(R-a)/\lambda} \norm{\psi}
\end{equation}
with $x$ sufficiently near the origin $\abs{x}\le a$, uniformly in the sample
size $R$ and the energy $E\in\Delta$. 
\end{lemma}

\begin{proof}[Proof]
Use the equation
\begin{equation}
\psi(x)= \int(E-H_0-V_d) ^{-1}(x,y) V_0(y)\psi(y) dy
\end{equation}
and expand the resolvent in a Neumann-series.
\begin{equation}
\label{eq:neumann}
(E-H_0-V_d)^{-1} =  \sum_{n=0}^{\infty} \left((E-H_0)^{-1}
V_d \right)^{n}(E-H_0)^{-1},
\end{equation}
Consider a fixed $n$, and use the estimate \eqref{eq:R0} for each free
resolvent. This results in the following integrals to be estimated:
\begin{multline}
\int \Bigl(\prod_{i=1}^{n} C \abs{\ln(\abs{z_{i-1}-z_i}/\xi)}
e^{-\abs{z_{i-1}-z_i}/\xi}V_d(z_i)\Bigr) \times \\
C \abs{\ln(\abs{z_n-y}/\xi)} e^{-\abs{z_n-y}/\xi}
V_0(y)\abs{\psi(y)}  dz_1 \dots dz_n dy 
\end{multline}
with $z_0=x$, $z_{n+1}=y$. Taking out $V_d$, and spliting the
exponentials in $3$, this is estimated by
\begin{multline}
(C\norm{V_d}_{\infty})^n \sup_{z_1,\dots z_n} \exp(-\sum_{i=1}^{n+1}
\abs{z_{i-1}-z_i}/3\xi) \times \\
\Bigl(\int e^{-\abs{w}/3\xi}\abs{\ln(\abs{w}/\xi)}\Bigr)^n 
\sup_{z_1,\dots z_n} \int e^{-\abs{z_n-y}/3\xi}
\abs{\ln(\abs{z_n-y}/\xi)} \times \\  \exp(-\sum_{i=1}^{n+1}
\abs{z_{i-1}-z_i}/3\xi) V_0(y)\abs{\psi(y)} dy
\end{multline}
Now $\inf_{z_1,\dots z_n}\sum_{i=1}^{n+1} \abs{z_{i-1}-z_i} \ge \abs{x-y}$ and applying the Schwarz inequality to the last integral,
the bound moves to
\begin{multline}
 (\tilde{C}\norm{V_d}_{\infty})^n e^{-\abs{x-y}/3\xi} 
\Bigl(\int e^{-2\abs{w}/3\xi} \abs{\ln(\abs{w}/\xi)}^2 dw\Bigr)^{1/2}
\times \\
\Bigl(\int e^{-2\abs{x-y}/3\xi} (V_0(y))^2 \abs{\psi(y)}^2dy \Bigr)^{1/2}
\end{multline}
If the potential does not increase too fast, the integral converges, and after 
summing over $n$, making the disorder small enough, the claim follows.
\end{proof}
The goal now is to prove the positivity of the current from the expression
derived in section \ref{sec:big}.
\begin{equation}
\begin{split}
I_{\varphi} & = \bigl(\psi,\frac{2}{2\pi r}
(\vec{p}-\vec{A})_{\varphi}\psi\bigr) \\ 
&=  \bigl(\psi,\frac{1}{2\pi B r} \partial_r V \psi\bigr) 
+\frac{2}{2\pi B}\bigl(\frac{1}{r}\partial_r \psi,\frac{1}{r}\partial_r
\psi\bigr) 
- \frac{1}{2\pi B} \bigl(\psi,\frac{2}{r^2} (\vec{p}-\vec{A})_{\varphi}^2\psi
\bigr).
\end{split}
\end{equation}
The first step is to eliminate the singularity at $r=0$ by replacing $\psi$
with $j\psi$, where $j$ is a cutoff at radius $a>0$ near the origin.
The error introduced by this replacement is
\begin{multline}
\label{eq:error}
 \bigl(\psi,\frac{1}{r} (p-A)_{\varphi}\psi\bigr) - 
 \bigl(j\psi,\frac{1}{r} (p-A)_{\varphi}j\psi\bigr) = \\ 
 \bigl((1-j)\psi,\frac{1}{r} (p-A)_{\varphi}j\psi\bigr) +
 \bigl(j\psi,\frac{1}{r} (p-A)_{\varphi}(1-j)\psi\bigr) +
 \bigl((1-j)\psi,\frac{1}{r} (p-A)_{\varphi}(1-j)\psi\bigr)
\end{multline}
Consider bounding the term 
\begin{equation}
\begin{split}
 \abs{\bigl((1-j)\psi,\frac{1}{r} (p-A)_{\varphi}(1-j)\psi\bigr)} & \le
\norm{\smash{\frac{1}{r^{3/4}} \psi}}_a
\norm{\smash{\frac{1}{r^{1/2}}(p-A)_{\varphi}\psi}}_a \\
& \le C e^{-R/\lambda} a^{1/4} \norm{\psi}
\norm{\smash{\frac{1}{r}\psi}}^{1/2}_a 
\norm{(p-A)^2_{\varphi}\psi}_a^{1/2} \\
\le C e^{-3R/2\lambda} a^{1/2} \norm{\psi}^2
\end{split}
\end{equation}
where $\norm{\,\cdot\,}_a$ has its obvious meaning, and 
we have taken advantage of the fact the $r$ commutes with
$(p-A)_{\varphi}$ and that $\norm{\smash{(\vec{p}-\vec{A})^2_{\varphi}\psi}}$ 
can be bounded by the energy\footnote{This Kato-estimate for
  $(\vec{p}-\vec{A})^2_{\varphi}$ is not trivial, since radial and azimuthal
  part of the kinetic energy do not commute. The same kind of estimate in the
  half-plane geometry is needed in section \ref{sec:diric}.}.
The other terms in \eqref{eq:error} 
similarly decay exponentially with the sample size. 

Reviewing the calculation that lead to equation \eqref{eq:toll}, 
additional terms introduced by $j$ are found to be 
\begin{multline}
\bigl(j\psi, \frac{1}{2\pi B}i\frac{\hat B\times \vec{r}}{r^2}
(\vec{p}-\vec{A})\times \hat B [H,j]\psi\bigr) 
+ \bigl(\psi,[H,j]  \frac{1}{2\pi B}i\frac{\hat B\times \vec{r}}{r^2}
(\vec{p}-\vec{A})\times \hat B j\psi\bigr) \\ =
\bigl(j\psi, \frac{1}{2\pi B r} (-\partial_r) [H,j] \psi \bigr) +
\bigl(\psi, [H,j] \frac{1}{2\pi B r} (-\partial_r) j\psi\bigr)
\end{multline}
$[H,j] = -2j'\partial_r - j'' -j'/r$ has support for $r$ near $a$.
Organize the various terms so that either no radial derivative
is acting on $\psi$, or one radial derivative, or the expression
$\frac{1}{r}\partial_r r\partial_r$. Terms with one radial derivative are
estimated, for example, as
\begin{equation}
\begin{split}
\abs{\bigl(j\psi, j''\frac{1}{r} \partial_r j\psi\bigr)} & \le 
\norm{\smash{j''\frac{1}{r}j'\psi}}_a \norm{\partial_r \psi} \\
&\le \frac{C}{a^4} e^{-(R-a)/\lambda} \norm{\psi}^2,
\end{split}
\end{equation}
where $C$ contains the energy as bound for $\norm{\partial_r \psi}$.
The terms with two radial derivatives, such as
\begin{equation}
\bigl(j'j\frac{1}{r}\psi, \frac{1}{r} \partial_r r\partial_r \psi \bigr)
\end{equation}
are estimated similarly. Terms without radial derivative acting on $\psi$
are even easier.

Cutting off with $j$ thus introduces error terms that decay expontentially
with the sample size. 

From \eqref{eq:toll}, we now estimate
\begin{equation}
\abs{\bigl(j\psi,\frac{1}{r^2} (\vec{p}-\vec{A})_{\varphi}^2j\psi
\bigr)} \le \norm{\smash{\frac{1}{r^2}j\psi}} \norm{j
(\vec{p}-\vec{A})_{\varphi}^2\psi}
\end{equation}
The second factor is bounded by the energy. The first is split into a
part with the radial coordinate between $a$ and $R/2$, so that it decays as
\begin{equation}
\frac{1}{a^2} e^{-R/2\lambda}
\end{equation}
and a part from $R$ to $\infty$ which decays as $1/R^2$.
The positivity of 
\begin{equation}
\bigl(j\psi,\frac{1}{ r} \partial_r V j\psi\bigr) 
\end{equation}
is proved in a fashion very similar to the one in section \ref{sec:edge} by
introducing another cutoff function at the edge $r=R$\footnote{The cutoff at
  $r=a$ does not 
  significantly perturb the argument of section \ref{sec:edge} because $\psi$
  is exponentially small near the center.}.
The lower bound for the expression decays as $1/R$. If the sample is big
and the disorder small, the current is positive.



==> paper/poscomm.tex <==
If in a classical Hamiltonian system, one can show that for some orbit the
Poisson bracket of some coordinate $K$ with the Hamiltonian $H$
remains bounded away from zero, $\dot K = \{K,H\} \geq \alpha >0$, for all
times, one can conclude that the motion is delocalized over this coordinate. 
The quantum mechanical counterpart of this simple statement is the following:
Assume there exists a ``conjugate operator'' $A$, such that the commutator of
$A$ with the Hamiltonian is positive on some energy intervall $\Delta$
\begin{equation}
E_{\Delta}(H)\left[ H,iA \right] E_{\Delta}(H) \geq \alpha
E_{\Delta}(H)  
\label{eq:mouest} 
\end{equation}
with $\alpha > 0$, and where $E_{\Delta}(H)$ denotes the spectral projector of
$H$ on $\Delta$. Noting that if $\psi$ is an eigenstate of $H$ we have 
$\left(\psi,\left[H,iA\right]\psi\right)=0$ by the virial theorem, we can
conclude from \eqref{eq:mouest}
that $H$ can have no eigenvalue in the intervall $\Delta$. It was
first proved by Mourre \cite{mourre} that under additional assumptions 
of regularity of $H$ and its commutators with $A$, the spectrum of $H$ is
even purely absolutely continuous on $\Delta$.
Equation \eqref{eq:mouest} is termed a Mourre estimate. 

The necessary assumptions on $H$ have been subsequently relaxed considerably,
see, for example \cite{cycon} or, for even weaker assumptions, \cite{ABG}.
For the treatment of the problem with a smooth steep edge potential in section
\ref{sec:edge}, the original assumptions of Mourre 
are actually enough. Those are (see \cite{mourre}):
\begin{enumerate}
\renewcommand{\labelenumi}{(\roman{enumi})}
\renewcommand{\theenumi}{(\roman{enumi})}
\setlength{\parskip}{0cm}
\item \label{pcassum1} $H$ and $A$ are self-adjoint operators with domains
  $\De(H)$ and $\De(A)$. $\De(H)\cap\De(A)$ is a core for $H$.
\item \label{pcassum2} The unitary group $e^{iAa}$ generated by $A$
  leaves $\De(H)$ invariant and for all $\psi\in\De(H)$
\begin{equation*}
\sup_{\abs{a}<1}\norm{He^{iAa}\psi} < \infty
\end{equation*}
\item \label{pcassum3} The quadratic form $\left[H,iA\right]$ which is defined
  on $\De(H)\cap\De(A)$, is bounded below and closeable; the associated
  self-adjoint operator admits a domain containing $\De(H)$.
\item \label{pcassum4} The quadratic form $\bigl[[H,iA],iA\bigr]$
 is form-bounded by $\abs{H}^2$.
\end{enumerate}

Following Mourre's work, the main efforts have gone in the direction of
reducing the assumptions of regularity \ref{pcassum3} and \ref{pcassum4}.
We do not know of any results if the conjugate operator is not self-adjoint.
In the case of Dirichlet boundary conditions in section \ref{sec:diric}, we
will be in such a situation, and we will need several tricks to fit the
problem into a framework treated in \cite{sahbani}. Since a virial theorem
is also valid for non self-adjoint operators, we think that the conjugate
operator method might be extendable to those situation.

%For $s\in\R$, let $\Hi_s$ be the domain of $\abs{H}^s$, endowed with
%the graph-norm $\norm{\psi}_s=\norm{(\abs{H}+1)^{s/2}\psi}$. Then assume:
%\begin{enumerate}
%\setlength{\parskip}{0cm}
%\renewcommand{\labelenumi}{(\roman{enumi})}
%\renewcommand{\theenumi}{(\roman{enumi})}
%\item \label{pcassum1}  $\Hi_2\cap\De(A)$ is a core for $H$, that is, is dense
%  in $\Hi_2$.
%\item \label{pcassum2} The quadratic form $[H,iA]$, defined on ${\cal
%  D}(H)\cap\De(A)$ can be extended to a bounded operator from 
%  $\Hi_2$ to $\Hi_{-1}$.
%\item \label{pcassum3} The form $\bigl[[H,iA],iA\bigr]$, defined on
% $\De(H)\cap\De(A)$  
% can be extended to a bounded operator from $\Hi_2$ to $\Hi_{-2}$. 
%\item \label{pcassum4} There exists a self-adjoint operator $H_0$ with domain
%  $\De(H_0)=\De(H)$, so that $[H_0,iA]$ can be extended to a bounded operator 
%  from $\Hi_2$ to $\Hi$, and so that $\De(A)\cap\De(H_0 A)$ is a core for
%  $H_0$. 
%\end{enumerate}

%These assumptions can be relaxed significantly, see \cite{sahbani} and
%\cite{ABG}, and when we come to Dirichlet boundary conditions in section
%\ref{sec:diric}, it will be necessary to consider those
%more refined versions of the ``conjugate operator method''. 



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "pcqh"
%%% End: 


